Teaching LLMs Human-Like Editing of Inappropriate Argumentation via Reinforcement Learning

Editing human-written text has become a standard use case of large language models (LLMs), for example, to make one's arguments more appropriate for a discussion. Comparing human to LLM-generated edits, however, we observe a mismatch in editing strategies: While LLMs often perform multiple scattered edits and tend to change meaning notably, humans rather encapsulate dependent changes in self-contained, meaning-preserving edits. In this paper, we present a reinforcement learning approach that teaches LLMs human-like editing to improve the appropriateness of arguments. Our approach produces self-contained sentence-level edit suggestions that can be accepted or rejected independently. We train the approach using group relative policy optimization with a multi-component reward function that jointly optimizes edit-level semantic similarity, fluency, and pattern conformity as well as argument-level appropriateness. In automatic and human evaluation, it outperforms competitive baselines and the state of the art in human-like editing, with multi-round editing achieving appropriateness close to full rewriting.

==> acl26-edit-table-human-eval-quality.tex <==
\begin{table}[!t]
\centering
\small
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Con} & \textbf{Sim} & \textbf{Flu} & \textbf{HL} \\
\midrule
PPO$_{app=sim}$ & 3.72 & 3.11 & 3.43 & 3.95 \\
LLaMA & 4.18 & 4.20 & 4.31 & 4.32 \\
+ GRPO$_{full}$ (1$^{st}$) & \textbf{4.25} & \textbf{4.43} & \textbf{4.46} & \textbf{4.46} \\
\bottomrule
\end{tabular}
\caption{Human evaluation of revised arguments on a 5-point Likert scale. GRPO$_{full}$ (1$^{st}$) refers to GRPO$_{full}$ from Table~\ref{tab:ablation}. Metrics: Pattern Conformity (Con), Semantic Similarity (Sim), Fluency (Flu), and Human-Likeness (HL). Bold indicates best performance.}
\label{tab:human-eval-quality}
\end{table}


==> acl26-edit-table-human-eval-ranking.tex <==
\begin{table}[!t]
\centering
\small
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \textbf{1st} & \textbf{2nd} & \textbf{3rd} & \textbf{4th} & \textbf{Mean}$\downarrow$ & \textbf{Merit}$\uparrow$ \\
\midrule
PPO$_{app=sim}$ & 1 & 3 & 5 & \textbf{35} & 3.68 & 0.060 \\
LLaMA & 4 & 16 & \textbf{18} & 6 & 2.59 & 0.431 \\
+ GRPO$_{full}$ (1$^{st}$) & 4 & \textbf{20} & \textbf{18} & 2 & 2.41 & 0.529 \\
+ GRPO$_{full}$ (11$^{th}$) & \textbf{35} & 5 & 3 & 1 & \textbf{1.32} & \textbf{0.915} \\
\bottomrule
\end{tabular}
\caption{Bradley-Terry model rankings based on pairwise comparisons of revised arguments. GRPO$_{full}$ (1$^{st}$) refers to GRPO$_{full}$ from Table~\ref{tab:ablation}, while GRPO$_{full}$ (11$^{th}$) is the result after 11 rounds of iterative revision. Columns show counts of rank positions (1st-4th), mean rank, and merit score. Bold indicates highest value in each column (lowest for mean rank).}
\label{tab:human-eval-ranking}
\end{table}


==> human-likeness-example.tex <==
\begin{figure}[t!]
\centering
\small
\begin{tabular}{p{0.95\columnwidth}}
\toprule
\textbf{Original:} This paper makes really thoughtless but also quite offensive arguments. \\
\midrule
\textbf{Automatic Edits (Scattered, Interdependent):} \\
This paper makes \colorbox{pastelblue}{\textcolor{red}{\st{really thoughtless but also quite}} \textcolor{blue}{an}} offensive \colorbox{pastelyellow}{\textcolor{red}{\st{arguments}} \textcolor{blue}{argument}}. \\[0.5ex]
\textit{Applying individually fails:} \\
\quad \colorbox{pastelblue}{Edit 1} only: This paper makes {\color{red}\uwave{an offensive arguments}}. \\
\quad \colorbox{pastelyellow}{Edit 2} only: This paper {\color{red}\uwave{makes really thoughtless but also quite offensive argument}}. \\[0.5ex]
\textit{Both together succeed:} This paper makes an offensive argument. \\
\midrule
\textbf{Human-like Edit (Single, Self-contained):} \\
This paper makes \colorbox{pastelgray}{\textcolor{red}{\st{really thoughtless but also quite}} \textcolor{blue}{an}} \\
\colorbox{pastelgray}{\textcolor{black}{offensive} \textcolor{red}{\st{arguments}} \textcolor{blue}{argument}}. \\[0.5ex]
\textit{Result:} This paper makes an offensive argument. \\
\bottomrule
\end{tabular}
\vspace{-1ex}
\caption{Scattered, interdependent automatic edits fail when applied individually. A self-contained human-like edit encompasses all changes in one contiguous operation.}
\label{fig:human-likeness-example}
\end{figure}

